Lattice QCD with two dynamical flavors of domain wall quarks

We present results from the first large-scale study of two flavor QCD using domain wall fermions (DWF), a chirally symmetric fermion formulation which has proven to be very effective in the quenched approximation. We work on lattices of size 16^3x32, with a lattice cut-off of a^{-1}\approx 1.7 GeV, and dynamical (or sea) quark masses in the range m_{strange}/2 \simle m_{sea} \simle m_{strange}. After discussing the algorithmic and implementation issues involved in simulating dynamical DWF, we report on the low-lying hadron spectrum, decay constants, static quark potential, and the important kaon weak matrix element describing indirect CP violation in the Standard Model, B_K. In the latter case we include the effect of non-degenerate quark masses (m_s \neq m_u = m_d), finding B_K(MS-bar, 2 GeV) = 0.495(18).

==> text_sections/theoretical.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Section %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\section{From quenched to dynamical DWF simulation: theoretical prospective}
%\label{sec:theoretical}
%  File:  theoretical.tex
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifnum\theOutline=1
\begin{outline}
\item RG running vs quark flavors at short distance (at weak coupling).
      One anticipates rougher links at short distance in dynamical.
      In fact $\beta$ is smaller for same $a^{-1}$ for dynamical.
\item Briefely summarize quenched wilson and DBW2 
  (quenched differeces at sronger couping).
   With introducing DWF.
\item spacial correlation between topological density and spike 
\item topology changing configuration cause the spike.
\item Aoki phase limit, a bound for DWF at strong coupling.
\item Ealier  CU dynamical work.
\item Topological evolution in dynamical run. Express the expectation of
more mobility due to the roughness.
\item Stress the aim is $m_res$ to be small but not necessarily zero.
      c.f $\Omega$ argument.
\item Attempts to improve the chirality (e.g. 
Negative mass Wilson results. Adjoints action etc.)
\end{outline}
\fi

In this section we describe our theoretical expectation
for behaviors of dynamical domain wall fermions on lattice.

First we consider a comparison between quenched lattice ($N_F=0$) and
two flavor dynamical lattice ($N_F=2$) in a sufficiently weak couping regime, 
$a^{-1} \gg \Lambda_{QCD}$, where perturbation theory works well. 
The two lattices are matched 
The lattice spacing is set by some low energy dimensionful observable,
psuedo scalar decay constants for instance, thus the running couping constant
at the scale of lownergy $\mu \sim \Lambda_{QCD}$.


At intermediate coupling, we no longer reply on the perturbation 







% Local Variables:
% TeX-master: "../paper"
% End:

